On hyperlogarithms and Feynman integrals with divergences and many scales

It was observed that hyperlogarithms provide a tool to carry out Feynman integrals. So far, this method has been applied successfully to finite single-scale processes. However, it can be employed in more general situations. We give examples of integrations of three- and four-point integrals in Schwinger parameters with non-trivial kinematic dependence, involving setups with off-shell external momenta and differently massive internal propagators. The full set of Feynman graphs admissible to parametric integration is not yet understood and we discuss some counterexamples to the crucial property of linear reducibility. Furthermore we clarify how divergent integrals can be approached in dimensional regularization with this algorithm.

==> Graphs/makefile <==
.PHONY : clean all

%.dvi : %.tex
	latex "$<" -o "$@"

%.tex :
	echo "$(subst .tex,,$@)" | ~/Trees/treeformat > "$@"

%.eps : %.dvi
	dvips "$<" -E -o temp.eps
	~/Trees/epstool --copy --bbox temp.eps "$@"
	rm temp.eps

%.pdf : %.eps
#	ps2pdf -dEPSCrop "$<" "$@"
	ps2pdf "$<" tmp.pdf
	pdfcrop tmp.pdf "$@"
	rm tmp.pdf

todo : ../master.log
#	latex ../master.tex
	sed -n 's/! LaTeX Error: File `Trees\/\([^|]*\)'\'' not found\./\1\.pdf/p' < ../master.log > todo

all : todo $(shell cat todo)

clean :
	rm -f *.ps
	rm -f *.eps
	rm -f *.pdf
	rm -f *.tex
	rm -f *.dvi
	rm -f todo
	rm -f *.aux
	rm -f *.log




==> formulas/3_22.tex <==
\Phi\left( G_{3,22} \right)
&= \frac{\Gamma(1+3\varepsilon)\cdot p_1^{-6\varepsilon}}{(1-4\varepsilon)(1-5\varepsilon)} \sum_{n\geq -1} f_n \cdot \varepsilon^n
\quad\text{where}\quad
f_{-1} = 2\mzv{3}
\quad\text{and}\\
f_0 &=
\frac{6}{5}\mzv[2]{2}
+\frac{1}{z-\bar{z}} \left\{
\bar{\L}_{1,0,1,1}-\bar{\L}_{1,1,0,1}-\L_{1,0,1,1}+
\L_{1,1,0,1}-\L_{1,1,0,1}\bar{z}-\bar{\L}_{1,0,1,1}\bar{z}
-\bar{\L}_{1,0,1,1}z
\right.
\\&\quad
+\bar{\L}_{1,1,0,1}\bar{z}+\bar{\L}_{1,1,0,1}z+
\L_{1,0,1,1}\bar{z}-\bar{\L}_{1,1,0,0}z+\bar{\L}_{1,0,1,0}z+
\bar{\L}_{0,0,1,1}\bar{z}+\L_{1,1,0,0}\bar{z}
\\&\quad
-\L_{1,0,1,0}\bar{z}-
\bar{\L}_{0,1,0,1}\bar{z}-\L_{1}\bar{\L}_{1,1,0}+\L_{1}
\bar{\L}_{1,0,1}+\L_{1,1}\bar{\L}_{1,0}+\L_{1,1,0}\bar{\L}_{1}-
\L_{1,0,1}\bar{\L}_{1}
\\&\quad
-\L_{1,0}\bar{\L}_{1,1}
+6\mzv{3} \left( \L_{1}-\bar{\L}_{1}+\bar{\L}_{1}\bar{z}-\L_{1}z \right) 
-\L_{0,0,1,1}z
\\&\quad
+\L_{0,1,0,1}z+\L_{1,0,1,1}z-\L_{1,1,0,1}z+
\bar{\L}_{1,0,1,1}z\bar{z}+\L_{0,0,1,1}z\bar{z}-\bar{\L}_{1,1,0,1}z
\bar{z}
\\&\quad
-\L_{1,0,1,1}z\bar{z}-\bar{\L}_{1,0,1,0}z\bar{z}-\L_{0,1,0,1}z
\bar{z}-\bar{\L}_{0,0,1,1}\bar{z}z-\L_{1,1,0,0}\bar{z}z
\\&\quad
+\L_{1,0}\bar{\L}_{1,1}\bar{z}+\L_{1,0,1,0}\bar{z}z+\L_{1,0}\bar{\L}_{1,1}z+
\L_{1}\bar{\L}_{1,1,0}\bar{z}+\L_{1}\bar{\L}_{1,1,0}z
\\&\quad
-\L_{1,1}\bar{\L}_{1,0}\bar{z}-\L_{1}\bar{\L}_{1,0,1}z-\L_{1,1,0}\bar{\L}_{1}
\bar{z}-\L_{1,1,0}\bar{\L}_{1}z+\bar{\L}_{1,1,0,0}z\bar{z}
\\&\quad
+\L_{1,0,1}\bar{\L}_{1}\bar{z}+\bar{\L}_{0,1,0,1}\bar{z}z-\L_{1,1}\bar{\L}_{1,0}z
-\L_{1}\bar{\L}_{1,0,1}\bar{z}+\L_{1}\bar{\L}_{0,0,1}\bar{z}
\\&\quad
+\L_{0}\bar{\L}_{1,0,1}z+\L_{1,1,0}\bar{\L}_{0}\bar{z}+\L_{1,1}\bar{\L}_{0,0}
\bar{z}+\L_{0,1}\bar{\L}_{1,0}z-\L_{1,0,1}\bar{\L}_{0}\bar{z}
\\&\quad
-\L_{1,0}\bar{\L}_{0,1}\bar{z}-\L_{0,0,1}\bar{\L}_{1}z-\L_{0,0}\bar{\L}_{1,1}z-
\L_{0}\bar{\L}_{1,1,0}z+\L_{0,1,0}\bar{\L}_{1}z+\L_{0,1,0,0}\bar{z}z
\\&\quad
+\bar{\L}_{0,0,1,0}\bar{z}z-\L_{0,0,1,0}\bar{z}z-\L_{1}\bar{\L}_{0,1,0}
\bar{z}-\bar{\L}_{0,1,0,0}\bar{z}z+\L_{1,0,1}\bar{\L}_{1}z
\\&\quad
+\L_{1,1,0,1}z\bar{z}+\L_{1,0,1}\bar{\L}_{0}\bar{z}z+\L_{1}
\bar{\L}_{1,0,1}z\bar{z}+\L_{1,0}\bar{\L}_{0,1}\bar{z}z
\\&\quad
+\L_{1}\bar{\L}_{0,1,0}\bar{z}z+\L_{0,0,1}\bar{\L}_{1}z\bar{z}+\L_{0,0}
\bar{\L}_{1,1}z\bar{z}+\L_{1,1}\bar{\L}_{1,0}z\bar{z}
\\&\quad
+\L_{1,1,0}\bar{\L}_{1}z\bar{z}+\L_{0}\bar{\L}_{1,1,0}z\bar{z}-\L_{1,0,1}
\bar{\L}_{1}z\bar{z}-\L_{0,1,0}\bar{\L}_{1}z\bar{z}
\\&\quad
+\L_{0}\bar{\L}_{0,0,1}\bar{z}z-\L_{0,0}\bar{\L}_{0,1}\bar{z}z-\L_{0}
\bar{\L}_{0,1,0}\bar{z}z-\L_{0,0,1}\bar{\L}_{0}\bar{z}z
\\&\quad
+\L_{0,1}\bar{\L}_{0,0}\bar{z}z+\L_{0,1,0}\bar{\L}_{0}\bar{z}z-\L_{1,0}
\bar{\L}_{1,1}z\bar{z}-\L_{1}\bar{\L}_{0,0,1}\bar{z}z
\\&\quad
\left.
-\L_{0}\bar{\L}_{1,0,1}z\bar{z}-\L_{1,1,0}\bar{\L}_{0}\bar{z}z-\L_{1}
\bar{\L}_{1,1,0}z\bar{z}-\L_{1,1}\bar{\L}_{0,0}\bar{z}z
-\L_{0,1}\bar{\L}_{1,0}z\bar{z} 
\right\}


==> formulas/4loopvertex.tex <==
\Phi\left( \Delta_4 \right)
&=
\frac{4 p_1^{-2}}{\bar{z}-z} \left\{
	5\mzv{5} \left( \L_{0}\bar{\L}_{1}-\L_{1}\bar{\L}_{0}
+\bar{\L}_{1,0}-\bar{\L}_{0,1}-\L_{1,0}+\L_{0,1} \right)
	+3\mzv[2]{3} \left(\bar{\L}_{1}-\L_{1} \right)
\right.\nonumber\\&
 +2\mzv{3} \left( -\L_{1,0,1}\bar{\L}_{1}-\L_{0,1,1}\bar{\L}_{0}
 +\L_{0,1,1}\bar{\L}_{1}-\L_{1}\bar{\L}_{0,1,1}
 +\L_{1,0,1}\bar{\L}_{0}
 +\L_{0}\bar{\L}_{0,1,1}+\L_{1}\bar{\L}_{1,0,1}-\L_{0}\bar{\L}_{1,0,1}
 \right.\nonumber\\&\quad\qquad\left.
 +2\bar{\L}_{0,1,0,1}+\bar{\L}_{0,1,1,0}+2\L_{1,0,0,1}-\L_{0,1,1,0}
 -\bar{\L}_{1,0,1,0}-2\L_{0,1,0,1}+\L_{1,0,1,0}-2\bar{\L}_{1,0,0,1} \right)
	\nonumber\\&
-\bar{\L}_{1,0,0,1,1,0,1}
-\bar{\L}_{1,0,1,0,0,1,0}
+\bar{\L}_{1,0,1,0,0,1,1}
-\L_{1,0,\bar{z},0,1,1,0}
-\L_{1,0,\bar{z},1,0,0,1}
+\L_{1,0,\bar{z},1,1,0,0}
-\L_{0,1,\bar{z},0,0,1,1}
	\nonumber\\&
+\L_{0,1,\bar{z},0,1,1,0}
+\L_{0,1,\bar{z},1,0,0,1}
-\L_{0,1,\bar{z},1,1,0,0}
+\L_{1,0,\bar{z},0,0,1,1}
+\bar{\L}_{0,1,0,0,0,1,1}
-\bar{\L}_{0,1,0,0,1,1,0}
-\bar{\L}_{0,1,0,1,0,0,1}
	\nonumber\\&
+\bar{\L}_{0,1,0,1,1,0,1}
+\bar{\L}_{0,1,1,0,0,1,0}
-\bar{\L}_{0,1,1,0,0,1,1}
-\bar{\L}_{1,0,0,0,0,1,1}
+\bar{\L}_{1,0,0,0,1,1,0}
+\bar{\L}_{1,0,0,1,0,0,1}
+\L_{0,1,0,1,1,0,0}
	\nonumber\\&
-\L_{0,1,0,1,1,0,1}
-\L_{0,1,1,0,0,1,0}
+\L_{0,1,1,0,0,1,1}
-\L_{1,0,0,1,1,0,0}
+\L_{1,0,0,1,1,0,1}
+\L_{1,0,1,0,0,1,0}
-\L_{1,0,1,0,0,1,1}
	\nonumber\\&
+\L_{0}\bar{\L}_{0,1,1,0,0,1}
+\L_{0}\bar{\L}_{1,0,0,0,1,1}
-\L_{0}\bar{\L}_{1,0,1,0,0,1}
-\L_{1}\bar{\L}_{0,0,0,0,1,1}
+\L_{1}\bar{\L}_{0,0,0,1,1,0}
+\L_{1}\bar{\L}_{0,0,1,0,0,1}
	\nonumber\\&
-\L_{1}\bar{\L}_{0,0,1,1,0,0}
+\L_{1}\bar{\L}_{0,1,0,0,1,1}
-\L_{1}\bar{\L}_{0,1,1,0,0,1}
-\L_{1}\bar{\L}_{1,0,0,1,1,0}
+\L_{1}\bar{\L}_{1,0,1,1,0,0}
-\L_{0,1}\bar{\L}_{0,0,0,1,1}
	\nonumber\\&
+\L_{0,1}\bar{\L}_{0,0,1,1,0}
+\L_{0,1}\bar{\L}_{1,0,0,1,1}
-\L_{0,1}\bar{\L}_{1,0,1,1,0}
+\L_{1,0}\bar{\L}_{0,0,0,1,1}
-\L_{1,0}\bar{\L}_{0,0,1,1,0}
-\L_{1,0}\bar{\L}_{1,0,0,1,1}
\nonumber\\&
+\L_{0,1,\bar{z},1,0}\bar{\L}_{1,0}
-\L_{0,1,\bar{z},1,1}\bar{\L}_{0,0}
-\L_{1,0,0,1,1}\bar{\L}_{0,0}
+\L_{1,0,0,1,1}\bar{\L}_{1,0}
+\L_{1,0,1,0,0}\bar{\L}_{0,1}
-\L_{1,0,1,0,0}\bar{\L}_{1,1}
\nonumber\\&
+\L_{1,0,\bar{z},0,0}\bar{\L}_{1,1}
+\L_{0,1,1,0,0}\bar{\L}_{1,1}
-\L_{0,1,\bar{z},0,0}\bar{\L}_{1,1}
+\L_{0,1,\bar{z},0,1}\bar{\L}_{0,1}
-\L_{0}\bar{\L}_{0,1,0,0,1,1}
-\L_{1,0,\bar{z},0,1}\bar{\L}_{0,1}
\nonumber\\&
-\L_{1,0,\bar{z},1,0}\bar{\L}_{1,0}
+\L_{1,0,\bar{z},1,1}\bar{\L}_{0,0}
+\L_{0,1,0,1,1,0}\bar{\L}_{0}
-\L_{0,1,0,1,1,0}\bar{\L}_{1}
-\L_{0,1,1,0,0,1}\bar{\L}_{0}
+\L_{0,1,1,0,0,1}\bar{\L}_{1}
\nonumber\\&
-\L_{0,1,\bar{z},0,0,1}\bar{\L}_{1}
+\L_{0,1,\bar{z},0,1,1}\bar{\L}_{0}
+\L_{0,1,\bar{z},1,0,0}\bar{\L}_{1}
-\L_{0,1,\bar{z},1,1,0}\bar{\L}_{0}
-\L_{1,0,0,1,1,0}\bar{\L}_{0}
+\L_{1,0,0,1,1,0}\bar{\L}_{1}
\nonumber\\&
+\L_{1,0,1,0,0,1}\bar{\L}_{0}
-\L_{1,0,1,0,0,1}\bar{\L}_{1}
+\L_{1,0,\bar{z},0,0,1}\bar{\L}_{1}
-\L_{1,0,\bar{z},0,1,1}\bar{\L}_{0}
-\L_{1,0,\bar{z},1,0,0}\bar{\L}_{1}
+\L_{1,0,0,1}\bar{\L}_{1,0,1}
	\nonumber\\&
+\L_{1,0,1,0}\bar{\L}_{0,1,0}
-\L_{1,0,1,0}\bar{\L}_{1,1,0}
-\L_{1,0,\bar{z},0}\bar{\L}_{0,1,1}
+\L_{1,0,\bar{z},0}\bar{\L}_{1,1,0}
+\L_{1,0,\bar{z},1}\bar{\L}_{0,0,1}
+\L_{1,0,\bar{z},1,1,0}\bar{\L}_{0}
	\nonumber\\&
+\L_{1,0}\bar{\L}_{1,0,1,1,0}
+\L_{0,1,0}\bar{\L}_{0,0,1,1}
-\L_{0,1,0}\bar{\L}_{1,0,1,1}
-\L_{0,1,1}\bar{\L}_{0,1,0,0}
+\L_{0,1,1}\bar{\L}_{1,1,0,0}
-\L_{0,1,\bar{z}}\bar{\L}_{0,0,1,1}
	\nonumber\\&
+\L_{0,1,\bar{z}}\bar{\L}_{0,1,1,0}
+\L_{0,1,\bar{z}}\bar{\L}_{1,0,0,1}
-\L_{0,1,\bar{z}}\bar{\L}_{1,1,0,0}
-\L_{1,0,0}\bar{\L}_{0,0,1,1}
+\L_{1,0,0}\bar{\L}_{1,0,1,1}
+\L_{1,0,1}\bar{\L}_{0,1,0,0}
	\nonumber\\&
-\L_{1,0,1}\bar{\L}_{1,1,0,0}
+\L_{1,0,\bar{z}}\bar{\L}_{0,0,1,1}
-\L_{1,0,\bar{z}}\bar{\L}_{0,1,1,0}
-\L_{1,0,\bar{z}}\bar{\L}_{1,0,0,1}
+\L_{1,0,\bar{z}}\bar{\L}_{1,1,0,0}
+\L_{0,1,0,1}\bar{\L}_{0,0,1}
	\nonumber\\&
-\L_{0,1,0,1}\bar{\L}_{1,0,1}
-\L_{0,1,1,0}\bar{\L}_{0,1,0}
+\L_{0,1,1,0}\bar{\L}_{1,1,0}
+\L_{0,1,\bar{z},0}\bar{\L}_{0,1,1}
-\L_{0,1,\bar{z},0}\bar{\L}_{1,1,0}
-\L_{0,1,\bar{z},1}\bar{\L}_{0,0,1}
\nonumber\\&\left.
+\L_{0,1,\bar{z},1}\bar{\L}_{1,0,0}
-\L_{1,0,0,1}\bar{\L}_{0,0,1}
-\L_{1,0,\bar{z},1}\bar{\L}_{1,0,0}
+\L_{0,1,0,1,1}\bar{\L}_{0,0}
-\L_{0,1,0,1,1}\bar{\L}_{1,0}
-\L_{0,1,1,0,0}\bar{\L}_{0,1}
\right\} \nonumber\\
	&\quad + \bigo{\varepsilon}%


==> formulas/4pt_4loop_onshell_0.tex <==
\begin{split}%
f_0 &=
\tfrac{71}{16}\mzv{7}H_{{-1}}
 - \tfrac{1}{210}\mzv[3]{2}
\left(
2370H_{{-2}}
 - 1806H_{{-1,0}}
 + 11633H_{{-1,-1}}
\right)
 + \tfrac{1}{2}\mzv{5}
\Big(
12\mzv{2}H_{{-1}}
 + 44H_{{-1,-2}}
\\&\quad
 - 29H_{{-1,-1,0}}
 - 330H_{{-2,-1}}
 + 60H_{{-1,0,0}}
 + 150H_{{-2,0}}
 - 133H_{{-1,-1,-1}}
\Big)
 - 6\mzv[2]{3}
\left(
10H_{{-2}}
 + 3H_{{-1,-1}}
\right)
\\&\quad
 + \tfrac{1}{10}\mzv{3}
\Big(
900\mzv{2}H_{{-2,0}}
 - 410\mzv{2}H_{{-1,-1,-1}}
 + 273\mzv[2]{2}H_{{-1}}
 + 360\mzv{2}H_{{-1,0,0}}
 + 70\mzv{2}H_{{-1,-2}}
\\&\quad
 + 90\mzv{2}H_{{-1,-1,0}}
 - 1500\mzv{2}H_{{-2,-1}}
 + 60H_{{-1,-2,-1,-1}}
 - 60H_{{-1,-1,-2,-1}}
 - 10H_{{-1,-1,-1,-2}}
\\&\quad
 - 30H_{{-1,-1,-2,0}}
 + 40H_{{-1,-2,-2}}
 - 100H_{{-2,-1,-2}}
 - 230H_{{-1,-1,-1,0,0}}
 + 100H_{{-2,-2,-1}}
\\&\quad
 - 180H_{{-1,-1,-3}}
 - 20H_{{-1,-2,-1,0}}
 + 70H_{{-1,-3,-1}}
 - 600H_{{-2,-1,0,0}}
 - 160H_{{-1,-1,0,0,0}}
\\&\quad
 + 90H_{{-1,-3,0}}
 + 20H_{{-1,-2,0,0}}
\Big)
 - \tfrac{1}{10}\mzv[2]{2}
\Big(
54H_{{-1,-2,0}}
 - 180H_{{-1,-1,-1,-1}}
 - 27H_{{-1,-1,-2}}
\\&\quad
 + 30H_{{-2,-2}}
 + 37H_{{-1,-2,-1}}
 - 81H_{{-1,-3}}
 - 510H_{{-2,-1,0}}
 - 241H_{{-1,-1,-1,0}}
\\&\quad
 + 26H_{{-1,-1,0,0}}
 - 300H_{{-2,-1,-1}}
\Big)
 - \mzv{2}
\Big(
6H_{{-1,-2,-2,0}}
 - 2H_{{-1,-2,-1,-1,0}}
\\&\quad
 + 7H_{{-1,-2,0,0,0}}
 - 6H_{{-1,-2,-1,-2}}
 + 9H_{{-1,-3,-2}}
 + 60H_{{-2,-1,-3}}
 + 4H_{{-1,-3,0,0}}
\\&\quad
 + 10H_{{-2,-2,0,0}}
 + 12H_{{-1,-1,-4}}
 - 21H_{{-1,-3,-1,-1}}
 - 3H_{{-1,-3,-1,0}}
 + 6H_{{-1,-2,-1,0,0}}
\\&\quad
 - 6H_{{-1,-1,-2,0,0}}
 - 10H_{{-2,-1,-1,0,0}}
 - 6H_{{-1,-1,-3,0}}
 - 14H_{{-1,-1,-1,0,0,0}}
 - 20H_{{-2,-1,0,0,0}}
\\&\quad
 + 3H_{{-1,-1,-1,-2,-1}}
 - 10H_{{-1,-1,0,0,0,0}}
 - 30H_{{-2,-2,-1,-1}}
 - 12H_{{-1,-2,-2,-1}}
 - 20H_{{-2,-1,-2,0}}
\\&\quad
 - 9H_{{-1,-1,-2,-2}}
 + 30H_{{-2,-1,-2,-1}}
 + 21H_{{-1,-1,-1,-3}}
 - 6H_{{-1,-1,-1,-1,0,0}}
 - 7H_{{-1,-1,-1,-2,0}}
\\&\quad
 - 3H_{{-1,-1,-2,-1,0}}
 + 54H_{{-1,-1,-3,-1}}
 - 18H_{{-1,-2,-1,-1,-1}}
 + 18H_{{-1,-1,-2,-1,-1}}
\Big)
 + 10H_{{-2,-1,-2,0,0,0}}
\\&\quad
 + 5H_{{-1,-2,-1,0,0,0,0}}
 + 10H_{{-1,-3,-1,0,0,0}}
 - 20H_{{-2,-1,-3,0,0}}
 - 2H_{{-1,-2,-2,0,0,0}}
\\&\quad
 + 5H_{{-1,-1,-2,0,0,0,0}}
 + 7H_{{-1,-3,-1,-1,0,0}}
 + 6H_{{-1,-1,-1,-2,0,0,0}}
 + 6H_{{-1,-2,-1,-1,-1,0,0}}
 - H_{{-1,-1,-1,-2,-1,0,0}}
\\&\quad
 - 3H_{{-1,-3,-2,0,0}}
 - 12H_{{-1,-1,-3,0,0,0}}
 - 4H_{{-1,-1,-4,0,0}}
 - 18H_{{-1,-1,-3,-1,0,0}}
 - 6H_{{-1,-1,-2,-1,-1,0,0}}
\\&\quad
 + 4H_{{-1,-2,-2,-1,0,0}}
 + 10H_{{-2,-2,-1,-1,0,0}}
 - 3H_{{-1,-1,-2,-1,0,0,0}}
 + 10H_{{-2,-2,-1,0,0,0}}
 - 7H_{{-1,-1,-1,-3,0,0}}
\\&\quad
 + 8H_{{-1,-2,-1,-1,0,0,0}}
 + 3H_{{-1,-1,-2,-2,0,0}}
 + 2H_{{-1,-2,-1,-2,0,0}}
 - 10H_{{-2,-1,-2,-1,0,0}}
\end{split}


==> formulas/box2mass1off_1.tex <==
f_1 &=
 - 2S_{0,{\frac {m \left( -u+p \right) }{u+1}}}U_{-1}
 + 2S_{-u+p}U_{-1+m,-1}
 + 2S_{{\frac {m \left( -u+p \right) }{u+1}}}U_{-1}
 - P_{-1+m,-1+m}M_{0}
 + P_{0,-1+m}M_{0}
 - P_{-1+m}M_{0,0}
\nonumber\\&\quad
 - P_{-1+m}M_{0}
 - 2S_{-u+p,{\frac {m \left( -u+p \right) }{u+1}}}U_{-1}
 + 4S_{{\frac {m \left( -u+p \right) }{u+1}}}U_{-1,-1}
 - 2S_{{\frac {m \left( -u+p \right) }{u+1}}}U_{0,-1}
 - 2S_{{\frac {m \left( -u+p \right) }{u+1}}}U_{-1+m,-1}
 + 2S_{-u+p,p+1-m}M_{0}
 + 2S_{p+1-m}P_{-1,-1}
\nonumber\\&\quad
 - 2S_{{\frac {m \left( -u+p \right) }{u+1}}}P_{-1+m}M_{0}
 - U_{0,-1+m}M_{0}
 - 2S_{0,-m}M_{0}
 + 2S_{{\frac {m \left( -u+p \right) }{u+1}}}P_{0,-1}
 + 2S_{{\frac {m \left( -u+p \right) }{u+1}},-m}M_{0}
 - 2S_{{\frac {m \left( -u+p \right) }{u+1}},p+1-m}M_{0}
 - S_{p+1-m}M_{0,0}
\nonumber\\&\quad
 - S_{p+1-m,mp}P_{-1}
 + S_{mp}P_{-1+m}M_{0}
 + S_{p+1-m}P_{-1+m,-1}
 + S_{mp,p+1-m}M_{0}
 + 2S_{{\frac {m \left( -u+p \right) }{u+1}},p+1-m}P_{-1}
 + 2S_{-u+p}P_{-1+m}M_{0}
 - 4S_{{\frac {m \left( -u+p \right) }{u+1}}}P_{-1,-1}
\nonumber\\&\quad
 + 2S_{-u+p,{\frac {m \left( -u+p \right) }{u+1}}}P_{-1}
 + 2S_{{\frac {m \left( -u+p \right) }{u+1}}}U_{-1+m}M_{0}
 - 4S_{{\frac {m \left( -u+p \right) }{u+1}},{\frac {m \left( -u+p \right) }{u+1}}}P_{-1}
 - 2S_{-u+p,p+1-m}P_{-1}
 + 2S_{{\frac {m \left( -u+p \right) }{u+1}}}P_{-1+m,-1}
 - 2S_{-u+p}U_{-1+m}M_{0}
 + S_{p+1-m,p+1-m}P_{-1}
\nonumber\\&\quad
 + S_{-m}M_{0,0}
 + U_{-1+m,-1+m}M_{0}
 + U_{-1+m}M_{0,0}
 + S_{mp,mp}P_{-1}
 - S_{p+1-m}P_{-1+m}M_{0}
 + 2S_{-m,-m}M_{0}
 + 2S_{{\frac {m \left( -u+p \right) }{u+1}},mp}P_{-1}
\nonumber\\&\quad
 + 2S_{0,{\frac {m \left( -u+p \right) }{u+1}}}P_{-1}
 - 2S_{-u+p}P_{-1+m,-1}
 - 2S_{0,mp}P_{-1}
 - S_{mp}P_{-1+m,-1}
 - S_{p+1-m,-m}M_{0}
 - S_{mp,p+1-m}P_{-1}
 - S_{mp,-m}M_{0}
\nonumber\\&\quad
 - S_{p+1-m}P_{0,-1}
 - S_{p+1-m,p+1-m}M_{0}
 + 2S_{mp}P_{-1,-1}
 - S_{mp}P_{0,-1}
 + U_{-1+m}M_{0}
 - S_{p+1-m}M_{0}
 + S_{mp}P_{-1}
\nonumber\\&\quad
 + S_{-m}M_{0}
 - 2S_{{\frac {m \left( -u+p \right) }{u+1}}}P_{-1}
 + S_{p+1-m}P_{-1}
 + U_{-1}
 + S_{-m}
 - P_{-1}
 - U_{0,-1}
\nonumber\\&\quad
 + 2S_{{\frac {m \left( -u+p \right) }{u+1}},-m}
 - U_{-1+m,-1}
 + P_{-1+m,-1}
 - 2P_{-1,-1}
 + P_{0,-1}
 - S_{mp,-m}
 - S_{p+1-m,-m}
\nonumber\\&\quad
 - 2S_{0,-m}
 + 2U_{-1,-1}
 + 2S_{-m,-m}
 + 2S_{0,mp,-m}
 - 2S_{{\frac {m \left( -u+p \right) }{u+1}},p+1-m,-m}
 + 2P_{-1+m,-1,-1}
 - 2U_{-1+m,-1,-1}
\nonumber\\&\quad
 - P_{0,0,-1}
 - 2U_{-1,0,-1}
 + U_{-1+m,0,-1}
 + 2S_{-u+p,p+1-m,-m}
 - 2S_{p+1-m,-m,-m}
 + 2S_{mp,0,-m}
 - U_{-1+m,-1+m,-1}
\nonumber\\&\quad
 - 4S_{0,-m,-m}
 - S_{p+1-m,p+1-m,-m}
 + 2S_{-u+p,0,-m}
 - P_{0,-1+m,-1}
 + P_{-1+m,-1+m,-1}
 + 4S_{{\frac {m \left( -u+p \right) }{u+1}},-m,-m}
 - 4P_{-1,-1,-1}
\nonumber\\&\quad
 - 2S_{-m,0,-m}
 - 2S_{-u+p,{\frac {m \left( -u+p \right) }{u+1}},-m}
 + 2P_{0,-1,-1}
 - 2U_{0,-1,-1}
 + S_{p+1-m,mp,-m}
 - 4S_{{\frac {m \left( -u+p \right) }{u+1}},0,-m}
 + 4S_{-m,-m,-m}
\nonumber\\&\quad
 + 2S_{0,0,-m}
 + S_{mp,p+1-m,-m}
 - 2S_{mp,-m,-m}
 - 2S_{0,{\frac {m \left( -u+p \right) }{u+1}},-m}
 + U_{0,-1+m,-1}
 - 2S_{{\frac {m \left( -u+p \right) }{u+1}},mp,-m}
 + 4S_{{\frac {m \left( -u+p \right) }{u+1}},{\frac {m \left( -u+p \right) }{u+1}},-m}
\nonumber\\&\quad
 + 4U_{-1,-1,-1}
 + 2P_{-1,0,-1}
 - S_{mp,mp,-m}
 - P_{-1+m,0,-1}
 + U_{0,0,-1}
 + 4S_{{\frac {m \left( -u+p \right) }{u+1}},{\frac {m \left( -u+p \right) }{u+1}}}U_{-1}


==> formulas/boxdiag_2off_-1.tex <==

 - U_{0,-1+m}M_{0}
 + Q_{0,-1+m}M_{0}
 - S_{0,qm}Q_{-1}
 + P_{s+um-qm}Q_{0,-1}
 + P_{{\frac {us}{q}},s}S_{-m}
 + P_{s}S_{0,-m}
 - S_{m \left( -u+q \right) }U_{0,-1}
 + S_{m \left( -u+q \right) }Q_{0,-1}
 + U_{-1}S_{m \left( -u+q \right) ,{\frac {m \left( -u+q \right) }{u+1}}}
 + Q_{-1}S_{m \left( -u+q \right) ,qm}
 - Q_{-1}S_{m \left( -u+q \right) ,{\frac {m \left( -u+q \right) }{u+1}}}
 - Q_{-1}P_{s+um-qm,-{\frac {-us-s-um+qm}{q+1}}}
 - U_{-1}P_{u,um}
 - S_{-m}P_{s+um-qm,s}
 - P_{{\frac {us}{q}}}S_{{\frac {m \left( -u+q \right) }{u+1}},-m}
 - U_{-1}P_{{\frac {us}{q}},-{\frac {-us-s-um+qm}{q+1}}}
 - U_{-1}P_{s+um-qm,um}
 + U_{-1}P_{u,-m+u+1}
 + P_{u}U_{-1+m,-1}
 + S_{-m}P_{s+um-qm,-{\frac {-us-s-um+qm}{q+1}}}
 + U_{-1}P_{s+um-qm,-{\frac {-us-s-um+qm}{q+1}}}
 - S_{q}Q_{-1+m,-1}
 - P_{s+um-qm}S_{qm,-m}
 - Q_{-1}S_{q,-m+q+1}
 + P_{s+um-qm}S_{{\frac {m \left( -u+q \right) }{u+1}},-m}
 + Q_{-1}P_{{\frac {us}{q}},-{\frac {-us-s-um+qm}{q+1}}}
 + P_{{\frac {us}{q}}}S_{qm,-m}
 + U_{-1}P_{{\frac {us}{q}},um}
 - U_{-1}S_{0,{\frac {m \left( -u+q \right) }{u+1}}}
 + M_{0}S_{q,-m+q+1}
 + Q_{-1}S_{q,qm}
 - M_{0}P_{u,-m+u+1}
 - S_{-m}P_{{\frac {us}{q}},-{\frac {-us-s-um+qm}{q+1}}}
 + Q_{-1}S_{0,{\frac {m \left( -u+q \right) }{u+1}}}
 - P_{s+um-qm}S_{0,-m}
 - P_{s+um-qm}U_{0,-1}
 - P_{{\frac {us}{q}}}S_{{\frac {m \left( -u+q \right) }{u+1}}}U_{-1}
 + S_{q}Q_{-1+m}M_{0}
 - P_{u}U_{-1+m}M_{0}
 + P_{s+um-qm}S_{{\frac {m \left( -u+q \right) }{u+1}}}U_{-1}
 + P_{{\frac {us}{q}}}S_{{\frac {m \left( -u+q \right) }{u+1}}}Q_{-1}
 - P_{{\frac {us}{q}}}S_{qm}Q_{-1}
 - P_{s+um-qm}S_{{\frac {m \left( -u+q \right) }{u+1}}}Q_{-1}
 + P_{s+um-qm}S_{qm}Q_{-1}
 + P_{u,um,-m}
 + S_{q,-m+q+1,-m}
 - P_{u,-m+u+1,-m}
 + S_{0,qm,-m}
 + P_{s+um-qm,um,-m}
 + P_{{\frac {us}{q}},-{\frac {-us-s-um+qm}{q+1}},-m}
 + U_{0,-1+m,-1}
 + S_{q,0,-m}
 - P_{u,0,-m}
 - P_{s,0,-m}
 - Q_{0,-1+m,-1}
 - P_{s+um-qm,-{\frac {-us-s-um+qm}{q+1}},-m}
 + S_{m \left( -u+q \right) ,{\frac {m \left( -u+q \right) }{u+1}},-m}
 - S_{m \left( -u+q \right) ,0,-m}
 - S_{m \left( -u+q \right) ,qm,-m}
 + P_{s+um-qm,s,-m}
 - P_{{\frac {us}{q}},um,-m}
 + S_{0,0,-m}
 - P_{{\frac {us}{q}},s,-m}
 + P_{{\frac {us}{q}},0,-m}
 - S_{0,{\frac {m \left( -u+q \right) }{u+1}},-m}
 - S_{q,qm,-m}

==> formulas/diag2mass2off_-1.tex <==
f_{-1} &=
 - U_{0,-1+m}M_{0}
 + Q_{0,-1+m}M_{0}
 - S_{0,qm}Q_{-1}
 + P_{s+um-qm}Q_{0,-1}
 + P_{{\frac {us}{q}},s}S_{-m}
\nonumber\\&\quad
 + P_{s}S_{0,-m}
 - S_{m \left( -u+q \right) }U_{0,-1}
 + S_{m \left( -u+q \right) }Q_{0,-1}
 + U_{-1}S_{m \left( -u+q \right) ,{\frac {m \left( -u+q \right) }{u+1}}}
\nonumber\\&\quad
 + Q_{-1}S_{m \left( -u+q \right) ,qm}
 - Q_{-1}S_{m \left( -u+q \right) ,{\frac {m \left( -u+q \right) }{u+1}}}
 - Q_{-1}P_{s+um-qm,-{\frac {-us-s-um+qm}{q+1}}}
 - U_{-1}P_{u,um}
\nonumber\\&\quad
 - S_{-m}P_{s+um-qm,s}
 - P_{{\frac {us}{q}}}S_{{\frac {m \left( -u+q \right) }{u+1}},-m}
 - U_{-1}P_{{\frac {us}{q}},-{\frac {-us-s-um+qm}{q+1}}}
 - U_{-1}P_{s+um-qm,um}
\nonumber\\&\quad
 + U_{-1}P_{u,-m+u+1}
 + P_{u}U_{-1+m,-1}
 + S_{-m}P_{s+um-qm,-{\frac {-us-s-um+qm}{q+1}}}
 + U_{-1}P_{s+um-qm,-{\frac {-us-s-um+qm}{q+1}}}
 - S_{q}Q_{-1+m,-1}
\nonumber\\&\quad
 - P_{s+um-qm}S_{qm,-m}
 - Q_{-1}S_{q,-m+q+1}
 + P_{s+um-qm}S_{{\frac {m \left( -u+q \right) }{u+1}},-m}
 + Q_{-1}P_{{\frac {us}{q}},-{\frac {-us-s-um+qm}{q+1}}}
\nonumber\\&\quad
 + P_{{\frac {us}{q}}}S_{qm,-m}
 + U_{-1}P_{{\frac {us}{q}},um}
 - U_{-1}S_{0,{\frac {m \left( -u+q \right) }{u+1}}}
 + M_{0}S_{q,-m+q+1}
 + Q_{-1}S_{q,qm}
\nonumber\\&\quad
 - M_{0}P_{u,-m+u+1}
 - S_{-m}P_{{\frac {us}{q}},-{\frac {-us-s-um+qm}{q+1}}}
 + Q_{-1}S_{0,{\frac {m \left( -u+q \right) }{u+1}}}
 - P_{s+um-qm}S_{0,-m}
 - P_{s+um-qm}U_{0,-1}
\nonumber\\&\quad
 - P_{{\frac {us}{q}}}S_{{\frac {m \left( -u+q \right) }{u+1}}}U_{-1}
 + S_{q}Q_{-1+m}M_{0}
 - P_{u}U_{-1+m}M_{0}
 + P_{s+um-qm}S_{{\frac {m \left( -u+q \right) }{u+1}}}U_{-1}
\nonumber\\&\quad
 + P_{{\frac {us}{q}}}S_{{\frac {m \left( -u+q \right) }{u+1}}}Q_{-1}
 - P_{{\frac {us}{q}}}S_{qm}Q_{-1}
 - P_{s+um-qm}S_{{\frac {m \left( -u+q \right) }{u+1}}}Q_{-1}
 + P_{s+um-qm}S_{qm}Q_{-1}
\nonumber\\&\quad
 + P_{u,um,-m}
 + S_{q,-m+q+1,-m}
 - P_{u,-m+u+1,-m}
 + S_{0,qm,-m}
 + P_{s+um-qm,um,-m}
\nonumber\\&\quad
 + P_{{\frac {us}{q}},-{\frac {-us-s-um+qm}{q+1}},-m}
 + U_{0,-1+m,-1}
 + S_{q,0,-m}
 - P_{u,0,-m}
 - P_{s,0,-m}
\nonumber\\&\quad
 - Q_{0,-1+m,-1}
 - P_{s+um-qm,-{\frac {-us-s-um+qm}{q+1}},-m}
 + S_{m \left( -u+q \right) ,{\frac {m \left( -u+q \right) }{u+1}},-m}
 - S_{m \left( -u+q \right) ,0,-m}
\nonumber\\&\quad
 - S_{m \left( -u+q \right) ,qm,-m}
 + P_{s+um-qm,s,-m}
 - P_{{\frac {us}{q}},um,-m}
 + S_{0,0,-m}
 - P_{{\frac {us}{q}},s,-m}
\nonumber\\&\quad
 + P_{{\frac {us}{q}},0,-m}
 - S_{0,{\frac {m \left( -u+q \right) }{u+1}},-m}
 - S_{q,qm,-m}

